Revisiting Model-Agnostic Private Learning: Faster Rates and Active Learning

The Private Aggregation of Teacher Ensembles (PATE) framework is one of the most promising recent approaches in differentially private learning. Existing theoretical analysis shows that PATE consistently learns any VC-classes in the realizable setting, but falls short in explaining its success in more general cases where the error rate of the optimal classifier is bounded away from zero. We fill in this gap by introducing the Tsybakov Noise Condition (TNC) and establish stronger and more interpretable learning bounds. These bounds provide new insights into when PATE works and improve over existing results even in the narrower realizable setting. We also investigate the compelling idea of using active learning for saving privacy budget, and empirical studies show the effectiveness of this new idea. The novel components in the proofs include a more refined analysis of the majority voting classifier - which could be of independent interest - and an observation that the synthetic "student" learning problem is nearly realizable by construction under the Tsybakov noise condition.

==> app_gaussian_mech.tex <==
\section{Learning bound for PATE with Gaussian mechanism}

In this section, we provide a theoretical analysis of the version of PATE from \citet{papernot2017semi,papernot2018scalable} that uses Gaussian mechanism to release the aggregated teacher labels. We will focus on the setting assuming $\tau$-TNC. 
Thought this result is not our main contribution, we note that standard PATE is a practical algorithm and this is the first learning-theoretic guarantees of PATE.

\begin{theorem}[Utility guarantee of Algorithm \ref{alg-priv-agg-pate}]\label{thm:standard_pate_tnc}
	Assume the data distribution $\cD$ and the hypothesis class $\cH$ obey the Tsybakov noise condition with parameter $\tau$, then with probability at least $1-\gamma$, there exists universal constant $C$ such that the output $\hat{h}_S$ of  Algorithm~\ref{alg-priv-agg-pate} with parameter $K$ satisfying
	$$K = \frac{6\sqrt{\log(2n)}(\sqrt{m \log(1/\delta)} + \sqrt{m \log(1/\delta) + \epsilon m})}{\epsilon}$$
	obeys that 
	$$
	\mathtt{Err}(\hat{h}^S) - \mathtt{Err}(h^*) \leq \tilde{O}\bigg(\frac{d}{m} + \Big( \frac{d\sqrt{m}}{n\epsilon}\Big)^\frac{\tau}{2-\tau}\bigg).
	$$
	Specifically, in the realizable setting, then it follows that
	$$
	\mathtt{Err}(\hat{h}^S) - \mathtt{Err}(h^*) \leq \tilde{O}\Big(\frac{d}{m} + \frac{d\sqrt{m}}{n\epsilon}\Big).
	$$
\end{theorem}
\begin{proof}
	By the triangular inequality of the $0-1$ error,
	\begin{align}
	\mathtt{Err}(\hat{h}^S) - \mathtt{Err}(h^*)&\leq \Dis(\hat{h}^S,h^*)\nonumber\\
	&\leq \Dis(\hat{h}^S, \tilde{h}^\texttt{priv}) + \Dis(\tilde{h}^\texttt{priv}, h^*)\nonumber\\
	&\leq 2 \Dis(\tilde{h}^\texttt{priv}, h^*) + 2\sqrt{\frac{(d + \log(4/\gamma))\Dis(\tilde{h}^\texttt{priv},h^*)}{m}} + \frac{4(d + \log(4/\gamma))}{m}\nonumber\\
	&\leq 4 \Dis(\tilde{h}^\texttt{priv},h^*) + \tilde{O} \Big(\frac{d}{m}\Big)\label{eq:tnc_pate_deriv1}
	\end{align}
	where the third line follows from the learning bound (Lemma \ref{lem-excess}) with $\tilde{h}^\texttt{priv}$ being the labeling function for the student dataset. The last line is due to $a + 2\sqrt{ab} + b \leq 2a + 2b$ for non-negative $a,b$.
	
	The remaining problem would be finding the upper bound of $\Dis(\tilde{h}^\mathtt{priv},h^*)$. First by Lemma~\ref{lem-tnc}, with probability at least $1-\gamma/2$, $\forall k \in[K]$ we have
	\begin{align*}
	\Dis(\hat{h}_k,h^*) \lesssim \eta^\frac{2}{2-\tau}\Big(\frac{dK\log(n/d)+ \log(2K/\gamma)}{n}\Big)^\frac{\tau}{2-\tau}.
	\end{align*}
	
	Next, conditioning on the teachers, $\tilde{h}^\mathtt{priv}$ is independent for each input and well-defined for all input. Let $Z\sim \cN(0,\sigma^2)$. By Gaussian-tail bound and Markov's inequality,
	\begin{align*}
	&\ \Dis(\tilde{h}^\mathtt{priv},h^*) \\
	\leq&\ \P \Big[|Z| \leq \sigma\sqrt{2\log(2/\beta)}\Big] \P \bigg[\sum_{k=1}^K \1(\hat{h}_k(x)\neq h^*(x))  \geq K/2 - |Z|) \bigg| |Z| \leq \sigma\sqrt{2\log(2/\beta)} \bigg]\\
	&\quad + \P \Big[|Z| > \sigma\sqrt{2\log(2/\beta)} \Big] \\
	\leq&\ \frac{1}{K/2 - \sigma\sqrt{2\log(2/\beta)}}\sum_{k=1}^K\E[\1(\hat{h}_k(x)\neq h^*(x))] + \beta\\
	\leq&\ \frac{3}{K}  \sum_{k=1}^K \Dis(\hat{h}_k,h^*) +  \frac{1}{n}\\
	\lesssim&\ \eta^\frac{2}{2-\tau}\Big(\frac{dK\log(n/d)+ \log(2K/\gamma)}{n}\Big)^\frac{\tau}{2-\tau}.
	\end{align*}
	In the last line, we choose $\beta = 1/n$ and applied the assumption that $K \geq 6\sigma\sqrt{2\log (2n)}$.
	
	Note that our choice of $\sigma$ satisfies that
	\begin{align*}
	\sqrt{\frac{2m \log(1/\delta)}{\sigma^2}} + \frac{m}{2\sigma^2} = \epsilon.
	\end{align*}
	Solve the equation and we find that
	\begin{align*}
	\sigma = \frac{\sqrt{2 m \log(1/\delta)} + \sqrt{2 m \log(1/\delta) + 2\epsilon m}}{2\epsilon}.
	\end{align*}
	Therefore, the choice of $K$ is
	$$K = \frac{6\sqrt{\log(2n)}(\sqrt{m \log(1/\delta)} + \sqrt{m \log(1/\delta) + \epsilon m})}{\epsilon} = \tilde{O}\Big(\frac{\sqrt{m}}{\epsilon}\Big),
	$$
	where $\epsilon$ is assumed to be small.
% 	\yw{For the above to be true, an additional assumption that says $\sqrt{m}/\epsilon$ dominates is needed, for instance if $\epsilon>1$, then perhaps $\sqrt{m/\epsilon}$ would be the dominating factor?  Either add an assumption that says $\epsilon$ is small or include both regimes in the bound (and in the table, and check for the same issues in all other theorems.)}
	Put everything together, and the excess risk bound is
	\begin{align*}
	\mathtt{Err}(\hat{h}^S) - \mathtt{Err}(h^*) \leq \tilde{O}\bigg(\frac{d}{m} + \Big(\frac{d\sqrt{m}}{n\epsilon}\Big)^\frac{\tau}{2-\tau}\bigg).
	\end{align*}
	
\end{proof}

\begin{remark}
When $m$ is sufficient large ($d/m < \Big(\frac{d\sqrt{m}}{n\epsilon}\Big)^\frac{\tau}{2-\tau}$), it suffices to use a subset of randomly chosen data points to optimize the bound and we obtain an excess risk bound of  $\tilde{O}\Big(\big(\frac{d^{3/2}}{n\epsilon}\big)^\frac{2\tau}{4-\tau} \Big)$. When $\tau=1$, this yields the $\frac{d}{(n\epsilon)^{2/3}}$ rate that matches \citet{bassily2018model}'s analysis of SVT-based PATE.  To avoid any confusions,  Gaussian mechanism-based PATE is still theoretically inferior comparing to SVT-based PATE as we established in Theorem~\ref{thm-ug-psq}.
	\end{remark}

==> app_related_work.tex <==
\section{Related Work}\label{sec-rw}
The literature on differentially private machine learning is enormous and it is impossible for us to provide a comprehensive summary. Thus, our discussion focuses on only a few theoretical aspects.

\subsection{Theory of Private Learning}
The learnability and sample complexity of private learning were studied under various models in \citep{kasiviswanathan2011can,beimel2013characterizing,beimel2016private,chaudhuri2011sample,bun2015differentially,wang2016learning,bassily2019limits}. The VC-classes were shown to be learnable when the either the hypothesis class or the data-domain is finite \citep{kasiviswanathan2011can}. \citet{beimel2013characterizing} characterizes the sample complexity of private learning in the realizable setting with a ``dimension'' that measures the extent to which we can construct a specific discretization of the hypothesis space that works for ``all distributions'' on data.  This dimension is often not possible when $\cH$ and $\cX$ are both continuous. Specifically, the problem of learning threshold functions on $[0,1]$ having VC-dimension of $1$ is not privately learnable \citep{chaudhuri2011sample,bun2015differentially}.

\subsection{Weaker Private Learning Models}
This setting of private learning was relaxed in various ways to circumvent this artifact. These include protecting only the labels \citep{chaudhuri2011sample,beimel2016private}, leveraging prior knowledge with a prior distribution \citep{chaudhuri2011sample}, switching to the general learning setting with Lipschitz losses \citep{wang2016learning}, relaxing the distribution-free assumption \citep{wang2016learning}, and finally the setting we consider in this paper --- when we assume the availability of an auxiliary public data \citep{bassily2018model,bassily2019limits}. Note that these settings are closely related to each other in that some additional information about the distribution of the data is needed.

\subsection{Private Learning with an Auxiliary Public Dataset}
The problem of private learning with access to an additional public data was formally studied in \citep{bassily2019limits}, which reveals an interesting ``theorem of the alternatives''-type result that says either a VC-class is learnable without an auxiliary public dataset, or we need at least $m = \Omega(d/\alpha)$ public data points. They also provide an upper bound that says $\tilde{O}(d/\alpha^2)$ private data and $\tilde{O}(d/\alpha)$ public data are sufficient to agnostically learn any classes with VC-dimension $d$ to $\alpha$-excess risk.  The algorithm however uses an explicit $\alpha$-net covering argument due to \citep{beimel2016private}, thus is not an efficient algorithm that is implementable. Our results are complementary in that we focuses on advancing the theoretical understanding of PATE towards more-refined data-dependent analysis, and to investigate the use of active learning. That said, Example~\ref{exp:voting_fail} implies that PATE does not enjoy the same agnostic learning bounds.

\subsection{Privacy-Preserving Prediction}
There is another line of work \citep{dwork2018privacy} that focuses on the related problem of ``privacy-preserving predictions'' which does not release the learned model (which we do), but instead privately answer one query $x$ (which we need to answer many, so as to train a model that can be released). While their technique can be used to obtain bounds in our setting, it often involves significantly worse rates. More recent work under this model \citep[see e.g.,][]{dagan2019pac,nandi2020privately} relies on the explicit $\alpha$-net construction due to \citep{beimel2016private}  (just like that in \citep{bassily2019limits}) which cannot be implemented efficiently, instead we reduce to the learning bounds of empirical risk minimization (in the passive learning case) or active learning oracles. So if we believe supervised learning is practically easy, the algorithm can be implemented (and has been) in practice \citep{papernot2017semi,papernot2018scalable}. 
%We believe analyzing the strengths and limitation of a practical algorithm is important and complementary to the search of information-theoretically optimal (but inefficient) algorithms that achieve the optimal rates.

%considered a reduction approach, which relies only on blackbox learners, so if we believe supervised learning is practically easy, the algorithm can be implemented (and has been!) in practice. 


%In fact, we have **cited Beimel et al. (2016)  and discussed in details** the limitation of algorithms based on this result in the related work section when discussing Alon, Bassily, Moran (2019) on “Limits of private learning with access to public data”, which Nandi and Bassily  (2019) builds upon.  In our discussion, we acknowledged the optimal rates these work obtained for fully agnostic learning, but we stated up front (even in the abstract) that we consider primarily under Tsybakov noise condition (which is an old and well-established setting in learning theory), and to explore the idea of active learning, which none of the cited work did.  We believe analyzing the strengths and limitation of a practical algorithm is important and complementary to the search of information-theoretically optimal (but inefficient) algorithms that achieve the optimal rates.



\subsection{Statistical Learning Theory}
The Tsybakov noise condition (TNC) \citep{mammen1999smooth,tsybakov2004optimal} is a natural and well-established condition in generalization theory that has long been used in the analysis of passive as well as active learning \citep{boucheron2005theory}. The Tsybakov noise condition is known to yield better convergence rates for passive learning \citep{hanneke2014theory}, and label savings for active learning \citep{zhang2014beyond}. However, the contexts under which we use these techniques are different. For instance, while we are making the assumption of the Tsybakov noise condition, the purpose is not for active learning, but rather to establish stability. When we apply active learning, it is for the synthetic learning problem with pseudo-labels that we release privately. To the best of our knowledge, we are the first that formally study these quantities in the theory of private learning. 
Lastly, active learning was considered for PATE learning in \citep{zhao2019improving}, which demonstrates the clear practical benefits of adaptively selecting what to label. We remain the first that provides theoretical analysis with provable learning bounds.

% \blue{Chong: do we need related work on active learning?}

% \yw{We have discussed active learning above in ``statistical learning theory'', haven't we? In the rebuttal, Kamalika provided some active learning references, which demonstorates that TNC is a well-established concepts. Please take a look and incorporate the relevant parts in the above.}

==> app_svt_and_standard_pate.tex <==
\section{Deferred proofs of stated technical results}\label{sec-proof-for-completeness}

We have provided most proofs in the paper. In this section, we provide the privacy analysis as well as reproving the results of \citet{bassily2018model} in our notation so that it becomes clear where the improvement is coming from.

\begin{theorem}[Restatement of Theorem \ref{thm-pg-agg}]
	Algorithm~\ref{alg-priv-agg-pate}~and~\ref{alg-priv-agg} are both ($\epsilon,\delta$)-DP.
\end{theorem}

The proof for Algorithm~\ref{alg-priv-agg-pate} follows straightforwardly from Gaussian mechanism because the number of ``teachers'' who predict $1$ will have a global sensitivity of $1$. The proof for Algorithm~\ref{alg-priv-agg} is more delicate. It follows the arguments in the proof of Theorem 3.6 of  \citet{bassily2018arxiv} for the most part, which combines the \emph{sparse vector technique} (SVT)  \citep{hardt2010multiplicative} with the \emph{distance to stability} approach from  \citet{thakurta2013differentially}. The only difference in the stated result here is that we used the modern CDP approach to handle the composition which provides tighter constants.

\begin{proof}
	First note that the global sensitivity (Definition \ref{def-global-sen}) of the vote count is $1$. Algorithm~\ref{alg-priv-agg-pate} is a straightforward adaptive composition of $\ell$ Gaussian mechanisms (Lemma \ref{lem-gau}), which satisfies  $\frac{\ell}{2\sigma^2}$-zCDP. By Lemma~\ref{lem:cdp2dp}, we get that the choice of $\sigma$ gives us ($\epsilon,\delta$)-differential privacy.
	
	Let us now address Algorithm~\ref{alg-priv-agg}. First note that $\mathrm{margin}(x_j)$ as a function of the input dataset $D$ has a global sensitivity of $2$ for all $x_j$, thus $\mathrm{dist}_j$ has a global sensitivity of $1$.
	Following the proof of Theorem 3.6 of  \citet{bassily2018arxiv}, Algorithm~\ref{alg-priv-agg} can be considered a composition of Sparse Vector Technique (SVT) (Algorithm \ref{alg-svt}), which outputs a binary vector of $\{\perp,\top\}$ indicating the failures and successes of passing the screening by SVT, and the distance-to-stability mechanism (Algorithm \ref{alg-dist-ins}) which outputs $\{\hat{h}^{\mathtt{agg}}(x_j)\}$ for all coordinates where the output is $\perp$.
	Check that the length of this binary vector is random and is between $T$ and $\ell$. The  number of $\top$ is smaller than $T$. If $\{\hat{h}^{\mathtt{agg}}(x_j)\}$ is not revealed, then this would be the standard SVT, and the challenge is to add the additional outputs.
	
	The key trick of the proof inspired from the privacy analysis (Lemma \ref{lem-pg-dist-ins}) of the distance-to-stability is to discuss the two cases. In the first case, assume for all $j$ such that the output is $\perp$, $\hat{h}^{\mathtt{agg}}(x_j)$ remains the same over $D,D'$, then adding $\hat{h}^{\mathtt{agg}}(x_j)$ to the output obeys $0$-DP; in the second case, assume that there exists some $j$ where we output $\perp$ such that, $\hat{h}^{\mathtt{agg}}(x_j)$ is different under $D$ and $D'$, then for all these $j$ we know that $\mathrm{dist}_j = 0$ for both $D$ and $D'$. By the choice of $\lambda, w$, we know that the second case happens with probability at most $\delta/2$ using the tail of Laplace distribution and a union bound over all $\ell+T$ independent Laplace random variables. 
	Note that this holds uniformly over all possible adaptive choices of the nature, since this depends only on the added noise.
	
	Conditioning on the event that the second case do not happen, the output of the algorithm is only the binary vector of $\{\perp,\top\}$ from SVT. The SVT with cutoff $T$ is an adaptive composition of $T$ SVTs with cutoff$=1$. By our choice of parameter $\lambda$, each such SVT with cutoff$=1$ obeys pure-DP with privacy parameter $2/\lambda$, hence also satisfy CDP with parameter $2/\lambda^2$ by Proposition~1.4 of  \citet{bun2016concentrated}.
	Composing over $T$ SVTs, we get a CDP parameter of $2T/\lambda^2$. By Proposition~1.3 of  \citet{bun2016concentrated} (Lemma~\ref{lem:cdp2dp}), we can convert CDP to DP. The choice of $\lambda$ is chosen such that the composed mechanism obeys $(\epsilon,\delta/2)$-DP.  Combining with the second case above, this establishes the $(\epsilon,\delta)$-DP of Algorithm~\ref{alg-priv-agg}.
\end{proof}



\begin{theorem}[Restatement of Theorem \ref{thm-ug-bassily}] \label{thm:reproving_bassilyetal}
	Set
	$$T = 3(\E[\varepsilon(\hat{h}_1)] m + \sqrt{m\log(m/\beta)/2}),$$
	$$K = O \Big(\frac{\log(mT / \min(\delta,\beta))\sqrt{T\log(1/\delta)}}{\epsilon}\Big).$$ Let $\hat{h}^S$ be the output of Algorithm~\ref{alg-psq} that uses Algorithm~\ref{alg-priv-agg} for privacy aggregation. With probability at least $1-\beta$ (over the randomness of the algorithm and the randomness of all data points drawn iid), we have
	$$\varepsilon(\hat{h}^S) \leq  \tilde{O}\Big(\frac{d^2m \log(1/\delta)}{n^2\epsilon^2}  + \sqrt{\frac{d}{m}}\Big)$$
	for the realizable case, and
	$$\varepsilon(\hat{h}^S) \leq  13\varepsilon(h^*) +  \tilde{O}\Big(\frac{m^{1/3}d^{2/3}}{n^{2/3}\epsilon^{2/3}}  + \sqrt{\frac{d}{m}}\Big)$$
	for the agnostic case. 
\end{theorem}

\begin{proof}
The analysis essentially follows the proof of Theorem~\ref{thm-ug-psq} by replacing $h^*$ with $y$. First, by Hoeffding's inequality, with probability $1-\beta$ over the teacher data points, the total number of mistakes made by each teacher classifier is at most $m\E[\varepsilon(\hat{h}_1)] + \sqrt{m\log(m/\beta)/2}$, which is $B$ in Lemma \ref{lem:pigeon_hole}. Then following Lemma \ref{lem:pigeon_hole}, by choose $T=3B=3(m\E[\varepsilon(\hat{h}_1)] + \sqrt{m\log(m/\beta)/2})$, we ensure that the majority voting classifiers are correct and have high margin in at least $m-T$ examples.

\noindent\textbf{In the realizable setting.} Since $\varepsilon(h^*)=0$ and by standard statistical learning theory in the realizable case (Lemma \ref{lem-excess}), for each teacher classifier $\hat{h}_k$ we have
\begin{align*}
\varepsilon(\hat{h}_k) \leq 4\frac{d \log(n/K) + \log(4/\gamma)}{n/K}.
\end{align*}
Substitute our choice of $K=\tilde{O}(\sqrt{T\log(1/\delta)}/\epsilon)$ as in Lemma~\ref{lem:utility_svt} we get that w.h.p.
\begin{align*}
\varepsilon(\hat{h}_k) \leq \tilde{O}\Big(\frac{d\sqrt{T\log(1/\delta)}}{n\epsilon}\Big).
\end{align*}
Plug in the bound into our choice of $T=3(m\E[\varepsilon(\hat{h}_1)] + \sqrt{m\log(m/\beta)/2})$, we get 
\begin{align*}
T\leq \tilde{O}\Big(\frac{dm\sqrt{T\log(1/\delta)}}{n\epsilon}+\sqrt{\frac{m\log(m/\beta)}{2} }\Big).
\end{align*}
By solving the quadratic inequality, we get that $T$ obeys
$$
T \leq \tilde{O}\Big(\frac{d^2m^2\log(1/\delta)}{n^2\epsilon^2} + \sqrt{m} \Big).
$$
Recall that this choice of $K$ and $T$ ensures that Algorithm~\ref{alg-priv-agg} will have at most $T$ unstable queries during the $m$ rounds, which implies that with high probability, the privately released pseudo-labels to those ``stable'' queries are the same as the corresponding true labels.
%By the fact that this choice of $T$ guarantees the completion of  the  pseudo-labels of the Algorithm~\ref{alg-priv-agg} has a small error rate in labeling all student data $x_1,...,x_m$.

Now the next technical subtlety is to deal with the dependences in the student learning problem created by the pseudo-labels via a reduction to an ERM learner.  
By the standard Hoeffding-style uniform convergence bound (Lemma \ref{lem-dis-emp}),
\begin{align}
\varepsilon(\hat{h}^S) \leq&\  \hat{\varepsilon}(\hat{h}^S) + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\nonumber\\
\leq&\ \hat{\varepsilon}(\hat{h}^{\mathtt{priv}}) + \widehat{\Dis}(\hat{h}^{\mathtt{priv}}, \hat{h}^S) +  \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\nonumber\\
\leq&\ 2\hat{\varepsilon}(\hat{h}^{\mathtt{priv}})  +  \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\nonumber\\
\leq&\ \frac{2T}{m} +  \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\nonumber\\
=&\  \tilde{O}\Big(\frac{d^2m\log(1/\delta)}{n^2\epsilon^2} + \sqrt{\frac{d}{m}}\Big).\label{eq:thm_bassily_deriv1}
\end{align}
where we applied the triangular inequality in the second line, used that $\hat{h}^S$ is the minimizer of $\widehat{\Dis}(\hat{h}^{\mathtt{priv}}, \cdot)$ in the third line,  and then combined Lemma~\ref{lem:utility_svt} and Lemma~\ref{lem:pigeon_hole} to show that under the appropriate choice of $T$ and $K$ with high probability, $\hat{h}^{\mathtt{priv}}(x_j)$ correctly returns $y_j$ except for up to $T$ example. Finally, the choice of $T$ is substituted.


%
%Since $T$ is cutoff of unstable queries, and Algorithm~\ref{alg-priv-agg} completes all $m$ data points with high probability,  $\hat{\varepsilon}(\hat{h}^S) \leq T/m$. By the triangular inequality, 
%\begin{align*}
%\varepsilon(\hat{h}^S) \leq \hat{\varepsilon}(\hat{h}^S)  \frac{T}{m} + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big) \leq \tilde{O}\Big(\frac{d^2m\log(1/\delta)}{n^2\epsilon^2} + \sqrt{\frac{d}{m}}\Big).
%\end{align*}

\noindent\textbf{In agnostic setting.} By Lemma \ref{lem-excess}, with high probability, for all teacher classifier $\hat{h}_k$ for $k=1,...,K$, we have
\begin{align*}
\varepsilon(\hat{h}_k) - \varepsilon(h^*) \leq \tilde{O}\Big(\sqrt{\frac{d \log(n/K) + \log(4/\gamma)}{n/K}}\Big).
\end{align*}
Substitute the choice of $K=\tilde{O}(\sqrt{T\log(1/\delta)}/\epsilon)$ from Lemma \ref{lem:utility_svt}, we get
\begin{align*}
\varepsilon(\hat{h}_k) \leq \varepsilon(h^*)+  \tilde{O}\Big(\frac{d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}}\Big).
\end{align*}
Plug in the above bound into our choice $T=3(m\E[\varepsilon(\hat{h}_1)] + \sqrt{m\log(m/\beta)/2})$, we get that
\begin{equation}\label{eq:thm_bassily_deriv2}
T \leq 3 m \varepsilon(h^*) + \tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}}\Big).
\end{equation}

Further, we can write
\begin{align}
T &\leq 2(3m \varepsilon(h^*) + \tilde{O}(\sqrt{m})) \cdot \mathbbm{1}\bigg(\tilde{O}\Big(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}}\Big) \leq \frac{T}{2}\bigg)\nonumber\\
&\quad + \bigg(2 \tilde{O}\Big(\frac{m d^{1/2}}{n^{1/2}\epsilon^{1/2}}\Big)\bigg)^{4/3}\cdot \mathbbm{1}\bigg(\tilde{O}\Big(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}}\Big) > \frac{T}{2}\bigg)\nonumber\\
&\leq 6m \varepsilon(h^*) + \tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m^{4/3} d^{2/3}}{n^{2/3}\epsilon^{2/3}}\Big),\label{eq:thm_bassily_deriv3}
\end{align}
where the first line talks about two cases of Inequality \eqref{eq:thm_bassily_deriv2}: (1) $T/2 \leq T - \tilde{O}(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}})\leq 3m \varepsilon(h^*) + \tilde{O}(\sqrt{m})$ if $\tilde{O}(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}}) \leq T/2$, and (2) $T^{3/4} \leq 2 \tilde{O}(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}})$ if $\tilde{O}(\frac{m d^{1/2}T^{1/4}}{n^{1/2}\epsilon^{1/2}}) > T/2$; The second line is due to the indicator function is always $\leq 1$.

% \yw{I added the wlog assumption and the the missing $\tilde{O}(\sqrt{m})$. How did you get the following expression? Did you solve a cubic equation and discussed the different roots or is there some simpler arguments that you used? The constant $3$ is important because we are stating the leading term of the analysis. }
% Solving the inequality for $T$, we get that
% \red{\begin{align*}
% T\leq 3 m \varepsilon(h^*)+\tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m^{4/3}d^{2/3}}{n^{2/3}\epsilon^{2/3}}\Big).
% \end{align*}}

Similar to the realizable case, now we apply a reduction to ERM. By the Hoeffding's style uniform convergence bound (implied by Lemma \ref{lem-dis-emp})
\begin{align*}
\varepsilon(\hat{h}^S) &\leq \hat{\varepsilon}(\hat{h}^S) + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\\
&\leq\hat{\varepsilon}(\hat{h}^{\mathtt{priv}}) + \widehat{\Dis}(\hat{h}^{\mathtt{priv}}, \hat{h}^S)   + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\\
&\leq \hat{\varepsilon}(\hat{h}^{\mathtt{priv}}) + \widehat{\Dis}(\hat{h}^{\mathtt{priv}}, \hat{h}_1)   + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\\ 
&\leq 2\hat{\varepsilon}(\hat{h}^{\mathtt{priv}}) + \hat{\varepsilon}(\hat{h}_1) + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\\ 
&\leq \frac{2T}{m}  + \varepsilon(h^*) + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big)\\
&\leq 13 \varepsilon(h^*)+\tilde{O}\Big(\frac{m^{1/3}d^{2/3}}{n^{2/3}\epsilon^{2/3}} + \sqrt{\frac{d}{m}}\Big).
\end{align*}
where the second and fourth lines use the triangular inequality of $0-1$ error, the third line uses the fact that $\hat{h}^S$ is the empirical risk minimizer of the student learning problem with labels $\hat{h}^{\mathtt{priv}}$ and the fact that $h_1\in\cH$. The second last line follows from the fact that in those stable queries $\hat{h}^{\mathtt{priv}}(x_j)$ outputs $y_j$, and a standard agnostic learning bound. Finally, in the last line, we obtain 
the stated result by substituting the upper bound of $T$ from  \eqref{eq:thm_bassily_deriv3}.
% \blue{Chong: I double-checked the proof, due to a calculation error, from inequality \eqref{eq:thm_bassily_deriv2}, I found I could not obtain
% \begin{align*}
% T &\leq 3 m \varepsilon(h^*)+\tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m^{4/3}d^{2/3}}{n^{2/3}\epsilon^{2/3}}\Big)
% \end{align*}
% and the result
% \begin{align}
% \varepsilon(\hat{h}^S) &\leq 7\varepsilon(h^*)+\tilde{O}\Big(\frac{m^{1/3}d^{2/3}}{n^{2/3}\epsilon^{2/3}} + \sqrt{\frac{d}{m}}\Big).\label{eq:t}
% \end{align}
% As discussed in Remark \ref{rmk:mislarge}, Inequality \eqref{eq:t} implies a $\tilde{O}(\frac{d^{3/5}}{n^{2/5}\epsilon^{2/5}})$ error bound, and the $\tilde{O}(\frac{d^{3/2}}{\alpha^{5/2}})$ sample complexity bound matches Theorem 4.7 of Bassily's paper.}
% \blue{
% Chong: But how to solve the inequality \eqref{eq:thm_bassily_deriv2}? The main difficulty lies in $T^{1/4}$. It's hard to solve a quartic inequality. I come up with two alternative approaches.
% The FIRST approach is using $T \leq m$. From \eqref{eq:thm_bassily_deriv2}, we can write
% \begin{align*}
% T\leq 3 m \varepsilon(h^*)+\tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m^{5/4}d^{1/2}}{n^{1/2}\epsilon^{1/2}}\Big).
% \end{align*}
% And the final stated result is
% \begin{align}
% \varepsilon(\hat{h}^S) \leq 7\varepsilon(h^*)+\tilde{O}\Big(\frac{m^{1/4}d^{1/2}}{n^{1/2}\epsilon^{1/2}} + \sqrt{\frac{d}{m}}\Big).\label{eq:t-m}
% \end{align}
% The SECOND approach is using $T^{1/4} \leq T^{1/2}$. From \eqref{eq:thm_bassily_deriv2}, we can write
% \begin{align*}
% T\leq 3 m \varepsilon(h^*)+\tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m d^{1/2}T^{1/2}}{n^{1/2}\epsilon^{1/2}}\Big).
% \end{align*}
% Solve the quadratic inequality, we have
% \begin{align*}
% T\leq 3 m \varepsilon(h^*)+\tilde{O}(\sqrt{m}) + \tilde{O}\Big(\frac{m^2 d}{n \epsilon}\Big).
% \end{align*}
% And the final stated result is
% \begin{align}
% \varepsilon(\hat{h}^S) \leq 7\varepsilon(h^*)+\tilde{O}\Big(\frac{md}{n \epsilon} + \sqrt{\frac{d}{m}}\Big).\label{eq:t0.25}
% \end{align}
% However, Inequality \eqref{eq:t-m} implies a $\tilde{O}(\frac{d^{1/2}}{n^{1/5}\epsilon^{1/5}})$ error bound and a $\tilde{O}(\frac{d^{5/2}}{\alpha^5})$ sample complexity bound. Inequality \eqref{eq:t0.25} implies a $\tilde{O}(\frac{d^{2/3}}{n^{1/3}\epsilon^{1/3}})$ error bound and a $\tilde{O}(\frac{d^2}{\alpha^3})$ sample complexity bound. Both of them don't match Theorem 4.7 of Bassily's paper.
% }
% \blue{Chong: from Theorem 4.7 of Bassily's paper, it seems Inequality \eqref{eq:t} is the right result. But I don't know how to obtain \eqref{eq:t}. Inequalities \eqref{eq:t-m} and \eqref{eq:t0.25} are worse bounds than \eqref{eq:t}. Are they okay to be reported in the paper?
% }
% \blue{What is the following commented out argument about seriously? I have seen these kind of errors in the proof throughout the paper. Always be conscious on what problem you are solving and what argument that you are applying in every line of logical derivation.}
% \red{
% Since $T$ is cutoff of unstable queries, $\hat{\varepsilon}(\hat{h}^S) \leq T/m$,
% \begin{align*}
% \varepsilon(\hat{h}^S) \leq \frac{T}{m} + \tilde{O}\Big(\sqrt{\frac{d}{m}}\Big) \leq 3 \varepsilon(h^*)+\tilde{O}\Big(\frac{m^{1/3}d^{2/3}}{n^{2/3}\epsilon^{2/3}} + \sqrt{\frac{d}{m}}\Big).
% \end{align*}
% }
\end{proof}


The results stated in the table are obtained by minimizing the bound by choosing a random subset of data points to privately release labels.



\section{Learning bound for PATE with Gaussian Mechanism}

In this section, we provide a theoretical analysis of the version of PATE from \citet{papernot2017semi,papernot2018scalable} that uses Gaussian mechanism to release the aggregated teacher labels. We will focus on the setting assuming $\tau$-TNC. 
Thought this result is not our main contribution, we note that standard PATE is a practical algorithm and this is the first learning-theoretic guarantees of PATE.

\begin{theorem}[Utility guarantee of Algorithm \ref{alg-priv-agg-pate}]\label{thm:standard_pate_tnc}
	Assume the data distribution $\cD$ and the hypothesis class $\cH$ obey the Tsybakov noise condition with parameter $\tau$, then with probability at least $1-\gamma$, there exists universal constant $C$ such that the output $\hat{h}_S$ of  Algorithm~\ref{alg-priv-agg-pate} with parameter $K$ satisfying
	$$K = \frac{6\sqrt{\log(2n)}(\sqrt{m \log(1/\delta)} + \sqrt{m \log(1/\delta) + \epsilon m})}{\epsilon}$$
	obeys that 
	$$
	\varepsilon(\hat{h}^S) - \varepsilon(h^*) \leq \tilde{O}\bigg(\frac{d}{m} + \Big( \frac{d\sqrt{m}}{n\epsilon}\Big)^\frac{\tau}{2-\tau}\bigg).
	$$
	Specifically, in the realizable setting, then it follows that
	$$
	\varepsilon(\hat{h}^S) - \varepsilon(h^*) \leq \tilde{O}\Big(\frac{d}{m} + \frac{d\sqrt{m}}{n\epsilon}\Big).
	$$
\end{theorem}
\begin{proof}
	By the triangular inequality of the $0-1$ error,
	\begin{align}
	\varepsilon(\hat{h}^S) - \varepsilon(h^*)&\leq \Dis(\hat{h}^S,h^*)\nonumber\\
	&\leq \Dis(\hat{h}^S, \tilde{h}^\texttt{priv}) + \Dis(\tilde{h}^\texttt{priv}, h^*)\nonumber\\
	&\leq 2 \Dis(\tilde{h}^\texttt{priv}, h^*) + 2\sqrt{\frac{(d + \log(4/\gamma))\Dis(\tilde{h}^\texttt{priv},h^*)}{m}} + \frac{4(d + \log(4/\gamma))}{m}\nonumber\\
	&\leq 4 \Dis(\tilde{h}^\texttt{priv},h^*) + \tilde{O} \Big(\frac{d}{m}\Big)\label{eq:tnc_pate_deriv1}
	\end{align}
	where the third line follows from the learning bound (Lemma \ref{lem-excess}) with $\tilde{h}^\texttt{priv}$ being the labeling function for the student dataset. The last line is due to $a + 2\sqrt{ab} + b \leq 2a + 2b$ for non-negative $a,b$.
	
	The remaining problem would be finding the upper bound of $\Dis(\tilde{h}^\mathtt{priv},h^*)$. First by Lemma~\ref{lem-tnc}, with probability at least $1-\gamma/2$, $\forall k \in[K]$ we have
	\begin{align*}
	\Dis(\hat{h}_k,h^*) \lesssim \eta^\frac{2}{2-\tau}\Big(\frac{dK\log(n/d)+ \log(2K/\gamma)}{n}\Big)^\frac{\tau}{2-\tau}.
	\end{align*}
	
	Next, conditioning on the teachers, $\tilde{h}^\mathtt{priv}$ is independent for each input and well-defined for all input. Let $Z\sim \cN(0,\sigma^2)$. By Gaussian-tail bound and Markov's inequality,
	\begin{align*}
	&\ \Dis(\tilde{h}^\mathtt{priv},h^*) \\
	\leq&\ \P \Big[|Z| \leq \sigma\sqrt{2\log(2/\beta)}\Big] \P \bigg[\sum_{k=1}^K \1(\hat{h}_k(x)\neq h^*(x))  \geq K/2 - |Z|) \bigg| |Z| \leq \sigma\sqrt{2\log(2/\beta)} \bigg]\\
	&\quad + \P \Big[|Z| > \sigma\sqrt{2\log(2/\beta)} \Big] \\
	\leq&\ \frac{1}{K/2 - \sigma\sqrt{2\log(2/\beta)}}\sum_{k=1}^K\E[\1(\hat{h}_k(x)\neq h^*(x))] + \beta\\
	\leq&\ \frac{3}{K}  \sum_{k=1}^K \Dis(\hat{h}_k,h^*) +  \frac{1}{n}\\
	\lesssim&\ \eta^\frac{2}{2-\tau}\Big(\frac{dK\log(n/d)+ \log(2K/\gamma)}{n}\Big)^\frac{\tau}{2-\tau}.
	\end{align*}
	In the last line, we choose $\beta = 1/n$ and applied the assumption that $K \geq 6\sigma\sqrt{2\log (2n)}$.
	
	Note that our choice of $\sigma$ satisfies that
	\begin{align*}
	\sqrt{\frac{2m \log(1/\delta)}{\sigma^2}} + \frac{m}{2\sigma^2} = \epsilon.
	\end{align*}
	Solve the equation and we find that
	\begin{align*}
	\sigma = \frac{\sqrt{2 m \log(1/\delta)} + \sqrt{2 m \log(1/\delta) + 2\epsilon m}}{2\epsilon}.
	\end{align*}
	Therefore, the choice of $K$ is
	$$K = \frac{6\sqrt{\log(2n)}(\sqrt{m \log(1/\delta)} + \sqrt{m \log(1/\delta) + \epsilon m})}{\epsilon} = \tilde{O}\Big(\frac{\sqrt{m}}{\epsilon}\Big),
	$$
	where $\epsilon$ is assumed to be small.
% 	\yw{For the above to be true, an additional assumption that says $\sqrt{m}/\epsilon$ dominates is needed, for instance if $\epsilon>1$, then perhaps $\sqrt{m/\epsilon}$ would be the dominating factor?  Either add an assumption that says $\epsilon$ is small or include both regimes in the bound (and in the table, and check for the same issues in all other theorems.)}
	Put everything together, and the excess risk bound is
	\begin{align*}
	\varepsilon(\hat{h}^S) - \varepsilon(h^*) \leq \tilde{O}\bigg(\frac{d}{m} + \Big(\frac{d\sqrt{m}}{n\epsilon}\Big)^\frac{\tau}{2-\tau}\bigg).
	\end{align*}
	
\end{proof}

\begin{remark}
When $m$ is sufficient large ($d/m < \Big(\frac{d\sqrt{m}}{n\epsilon}\Big)^\frac{\tau}{2-\tau}$), it suffices to use a subset of randomly chosen data points to optimize the bound and we obtain an excess risk bound of  $\tilde{O}\Big(\big(\frac{d^{3/2}}{n\epsilon}\big)^\frac{2\tau}{4-\tau} \Big)$. When $\tau=1$, this yields the $\frac{d}{(n\epsilon)^{2/3}}$ rate that matches \citet{bassily2018model}'s analysis of SVT-based PATE.  To avoid any confusions,  Gaussian mechanism-based PATE is still theoretically inferior comparing to SVT-based PATE as we established in Theorem~\ref{thm-ug-psq}.
	\end{remark}
